Solving the TTC 2011 Compiler Optimization Case with GROOVE

This report presents a partial solution to the Compiler Optimization case study using GROOVE. We explain how the input graphs provided with the case study were adapted into a GROOVE representation and we describe an initial solution for Task 1. This solution allows us to automatically reproduce the steps of the constant folding example given in the case description. We did not solve Task 2.

==> eptcsdata.tex <==
\providecommand{\firstpage}{126}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.11}{10.4204/EPTCS.74.11}}
\pdfoutput=1

